HumanTOMATO: Text-aligned Whole-body Motion Generation

This work targets a novel text-driven whole-body motion generation task, which takes a given textual description as input and aims at generating high-quality, diverse, and coherent facial expressions, hand gestures, and body motions simultaneously. Previous works on text-driven motion generation tasks mainly have two limitations: they ignore the key role of fine-grained hand and face controlling in vivid whole-body motion generation, and lack a good alignment between text and motion. To address such limitations, we propose a Text-aligned whOle-body Motion generATiOn framework, named HumanTOMATO, which is the first attempt to our knowledge towards applicable holistic motion generation in this research area. To tackle this challenging task, our solution includes two key designs: (1) a Holistic Hierarchical VQ-VAE (aka H$^2$VQ) and a Hierarchical-GPT for fine-grained body and hand motion reconstruction and generation with two structured codebooks; and (2) a pre-trained text-motion-alignment model to help generated motion align with the input textual description explicitly. Comprehensive experiments verify that our model has significant advantages in both the quality of generated motions and their alignment with text.

==> sec/intro-notusethis.tex <==
\section{Introduction}


With the rapid development of Artificial Intelligence Generated Content, there is an explosion of huge demand for generating high-quality 3D human motions to be labor-saving in many industry scenarios, such as games, films, anime, and robotics. 
%
Generating motions with textual description is a natural interaction way. The text-driven motion generation task targets generating vivid and diverse motions that closely align with the given text semantics. 
%
With the rapid progress of generative models (\textit{e.g.}, motion diffusion models~\citep{mdm2022human,mld,motiondiffuse}) to boost the diversity and quality of generated motions, this area has been increasingly active~\citep{zhu2023human}.
%

However, existing text-driven motion generation methods still face two intractable difficulties. 
(1) Delicate whole-body motion generation with fine-grained reconstruction among body, hand, and face motions coherently is under-explored. 
%
For instance, when the user describes that ``\texttt{a person is \underline{immersed} in playing the \underline{piano}}.", existing models may generate ``\texttt{a person is playing \underline{drums} \underline{expressionlessly}, while the fingers remain \underline{unchanged}}.". 
%
(2) Text-motion misalignment. Motions contain dynamic diversity and ambiguity, and hierarchical body-part relations. 
%

To tackle the above issues, this work explores how to generate text-aligned whole-body motions effectively. 
%
Due to cross-modality challenges and high-dimensional motion data, we take a two-stage framework by motion reconstruction first and then learn the alignment between motion latent and text, like T2M-GPT~\citep{t2m-gpt}. 
%
Our framework, named \ModelName, comes with three key designs to make the two-stage model generate high-quality, diverse, and text-aligned whole-body motions.
%
First, for motion reconstruction, previous works adopt the vanilla Vector Quantized Variational Autoencoder (VQ-VAE) for motion with only one codebook, making the motion representation capability limited and incurring the codebook collapse problem, especially for whole-body motions. That is, directly replacing body-only motions with whole-body motions via the VQ-VAE will be futile, even though we double the codebook natively. The high-dimension fine-grained hand gestures and diverse body motions make it hard to maintain both motion perceptual quality and abstract features at very low bitrates.
% 
Inspired by residual vector quantization~(\textit{aka} RVQ)~\citep{rvq, zeghidour2021soundstream} in recent rapid progresses in music generation~\citep{defossez2022highfi, copet2023simple}, we introduce a Holistic Hierarchical VQ-VAE (\textit{aka} H${}^{2}$VQ) for fine-grained body and hand motion reconstruction with two hierarchical structure codebooks (\textit{i.e.}, hand and body codebooks with hierarchical relations). Compared with doubling the size of the original codebook {\naive}ly, the proposed H${}^{2}$VQ can significantly reduce the motion reconstruction error effectively.
%

Second, for text-aligned motion generation, the way to encode the input text and provide the language embedding as a prior is quite important while less explored.
%
Existing methods either use Contrastive Language-Image Pre-Training (CLIP~\citep{clip,motionclip}) or Large Language Models (\textit{e.g.}, T5~\citep{todo}), lacking the understanding of motions. They fail to distinguish the motion sequentiality, directions, and dynamics.
%
Motivated by the text-to-motion retrieval task that incorporates a contrastive loss to bridge the gap of cross-modal latent spaces~\citep{petrovich2023tmr} in a global receptive field, we pre-train a text encoder and a whole-body motion encoder via the text-whole-body motion retrieval (\textit{aka} TMR) optimization objective to align text-motion explicitly.
% with a codes prediction module
Third, given a text, the WMR text encoder will output language embedding as a start token to predict discrete codes auto-regressively in our proposed Hierarchical-GPT. The codes contain body and hand tokens hierarchically. For each body-hand token, we put them into a Body-hand Decoder to generate body-hand poses sequentially. To make the Hierarchical-GPT predict whole-body motion precisely, we further introduce a text-motion alignment optimization goal via the language embedding and the body-hand motion embedding via the WMR motion encoder with the generated body-hand motion as inputs.
%
Finally, based on the textual descriptions of facial expressions, we use the facial conditional VAE (cVAE~\citep{todo}) to decode facial motions with the same length as body-hand motions. The generated body, hand, and face motions can be composed of whole-body motion.


Before delving into details, we carefully clarify our main contributions as follows:

\begin{itemize}
    \item {
        To the best of our knowledge, we propose the challenging \textbf{T}ext-driven wh\textbf{O}le-body \textbf{M}otion gener\textbf{AT}i\textbf{O}n task for the first time and design a model~(\textit{aka} \textbf{HumanTOMATO}) to generate vivid whole-body motions well aligned with the text.
    }
    \item {
        To tackle the challenging whole-body motion generation research problem, we introduce  H${}^{2}$VQ for fine-grained body and hand motion reconstruction precisely. Accordingly, we design a Hierarchical-GPT combined with facial cVAE to generate whole-body motions.
    }
    \item {
        To enhance the consistency and alignment between texts and whole-body motion, we pre-train text-motion-aligned encoders via a retrieval optimization objective to strongly calibrate the alignment between text and motion.
    }
    \item {
        % For evaluating the alignment between generated motions and given texts, 
        We propose more accurate and challenging metrics (\textit{WMR-R-Precision$^{(256)}$} and \textit{WMR-Matching-score}) to serve future work.
    }
\end{itemize}
% 
We evaluate our HumanTOMATO model on both whole-body and body-only motion generation benchmarks~\citep{lin2023motion, guo2022generating, plappert2016kit, babel} and answer four research questions on our main contributions. Experimental results demonstrate our generated motions are vivid, as well as good alignment with given texts.

